Spoken Language Intelligence of Large Language Models for Language Learning

People have long hoped for a conversational system that can assist in real-life situations, and recent progress on large language models (LLMs) is bringing this idea closer to reality. While LLMs are often impressive in performance, their efficacy in real-world scenarios that demand expert knowledge remains unclear. LLMs are believed to hold the most potential and value in education, especially in the development of Artificial intelligence (AI) based virtual teachers capable of facilitating language learning. Our focus is centered on evaluating the efficacy of LLMs in the realm of education, specifically in the areas of spoken language learning which encompass phonetics, phonology, and second language acquisition. We introduce a new multiple-choice question dataset to evaluate the effectiveness of LLMs in the aforementioned scenarios, including understanding and application of spoken language knowledge. In addition, we investigate the influence of various prompting techniques such as zero- and few-shot method (prepending the question with question-answer exemplars), chain-of-thought (CoT, think step-by-step), in-domain exampler and external tools (Google, Wikipedia). We conducted large-scale evaluation on popular LLMs (20 distinct models) using these methods. We achieved significant performance improvements compared to the zero-shot baseline in the practical questions reasoning (GPT-3.5, 49.1% -> 63.1%; LLaMA2-70B-Chat, 42.2% -> 48.6%). We found that models of different sizes have good understanding of concepts in phonetics, phonology, and second language acquisition, but show limitations in reasoning for real-world problems. Additionally, we also explore preliminary findings on conversational communication.

==> tables/slill-applied-answer-acc.tex <==
\begin{tabular}{ccc lllll }
\toprule
\bf Model & \bf Para. & \bf Prompt & \bf Pron.(174) & \bf Stre.(56) & \bf Brea.(20) & \bf Into.(38) & \bf Acc. \\
\midrule
GPT-4 & - & 3-shot & 72.4(126) & 64.3(36) & 70.0(14) & 68.42(26) & 73.1 \\
GPT-3.5-turbo & - & 3-shot & 51.7(90) & 50.0(28)  & 40.0(8)  & 44.7(17) & 53.5 \\
LLaMA2-Chat & 70B & 3-shot & 34.5(60) & 41.1(23) & 45.0(9) & 42.1(16) \\
Flan-UL2 & 20B & 3-shot & 35.6(61) & 55.4(31) & 35.0(7) & 52.6(20) & 44.5 \\
Flan-T5-XXL & 11B & 3-shot & 39.7(69) & 46.4(26) & 50.0(10) & 55.3(21) & 47.8 \\
\midrule 
GPT-4 & - & CoT & 77.6(135) & 73.2(41) & 75.0(15) & 71.1(27) & 0.0 \\
GPT-3.5-turbo & - & CoT & 56.3(98) & 46.4(26) & 50.0(10) & 36.8(14)  \\
LLaMA2-Chat & 70B & CoT & 41.4(72) & 44.6(25) & 55.0(11)  & 47.4(18) & 0.0 \\
Flan-UL2 & 20B & CoT & 29.3(51) & 51.8(29) & 20.0(4) & 42.1(16) & 0.0 \\
Flan-T5-XXL & 11B & CoT & 35.1(61) & 41.1(23) & 30.0(6) & 50.0(19) & 0.0 \\
\bottomrule
\addlinespace[0.1cm]
\multicolumn{8}{l}{\small{
\textsuperscript{1}Averaged using $k=100$ samples.
}}
\end{tabular}
